Non-kissing complexes and tau-tilting for gentle algebras

We interpret the support $\tau$-tilting complex of any gentle bound quiver as the non-kissing complex of walks on its blossoming quiver. Particularly relevant examples were previously studied for quivers defined by a subset of the grid or by a dissection of a polygon. We then focus on the case when the non-kissing complex is finite. We show that the graph of increasing flips on its facets is the Hasse diagram of a congruence-uniform lattice. Finally, we study its $\mathbf{g}$-vector fan and prove that it is the normal fan of a non-kissing associahedron.

==> figures/blossomingQuiver.tex <==
\begin{tikzpicture}
	  \node(T1) at (0,0) {
		\begin{tikzpicture}
    	\node[inner sep = 1pt] (a) at (1,3) {$\bullet$};
    	\node[inner sep = 1pt] (b) at (1,1) {$\bullet$};
    	\node[inner sep = 1pt] (c) at (2,2) {$\bullet$};
    	\node[inner sep = 1pt] (d) at (3,3) {$\bullet$};
    	\node[inner sep = 1pt] (e) at (4,2) {$\bullet$};
    	\node[inner sep = 1pt] (f) at (5,3) {$\bullet$};
    	\node[inner sep = 1pt] (g) at (5,1) {$\bullet$};
    	\node[inner sep = 1pt] (h) at (6,2) {$\bullet$};
    	\node[inner sep = 1pt] (i) at (7,3) {$\bullet$};
        \path [->, ultra thick] (a) edge (c);
        \path [->, ultra thick] (d) edge (c);
        \path [->, ultra thick] (d) edge (e);
        \path [->, ultra thick] (f) edge (e);
        \path [->, ultra thick] (f) edge (h);
        \path [->, ultra thick] (i) edge (h);
        \path [->, ultra thick] (c) edge (b);
        \path [->, ultra thick] (e) edge (g);
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=a--c--b};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=g--e--f};
	  \end{tikzpicture}};
	  \node(T2) at (7.5,0) {
		\begin{tikzpicture}
    	\node[inner sep = 1pt] (a) at (1,3) {$\bullet$};
    	\node[inner sep = 1pt] (b) at (1,1) {$\bullet$};
    	\node[inner sep = 1pt] (c) at (2,2) {$\bullet$};
    	\node[inner sep = 1pt] (d) at (3,3) {$\bullet$};
    	\node[inner sep = 1pt] (e) at (4,2) {$\bullet$};
    	\node[inner sep = 1pt] (f) at (5,3) {$\bullet$};
    	\node[inner sep = 1pt] (g) at (5,1) {$\bullet$};
    	\node[inner sep = 1pt] (h) at (6,2) {$\bullet$};
    	\node[inner sep = 1pt] (i) at (7,3) {$\bullet$};
    	\node (x1) at (.2,3.8) {};
    	\node (x2) at (.2,2.2) {};
    	\node (x3) at (.2,1.8) {};
    	\node (x4) at (.2,.2) {};
    	\node (x5) at (1.8,.2) {};
    	\node (x6) at (2.8,1.2) {};
    	\node (x7) at (3.2,1.2) {};
    	\node (x8) at (4.2,.2) {};
    	\node (x9) at (5.8,.2) {};
    	\node (x10) at (5.5,1.5) {};
    	\node (x11) at (5.5,1.5) {};
    	\node (x12) at (6.8,1.2) {};
    	\node (x13) at (7.8,2.2) {};
    	\node (x14) at (7.8,3.8) {};
    	\node (x15) at (6.2,3.8) {};
    	\node (x16) at (5.8,3.8) {};
    	\node (x17) at (4.2,3.8) {};
    	\node (x18) at (3.8,3.8) {};
    	\node (x19) at (2.2,3.8) {};
    	\node (x20) at (1.8,3.8) {};
        \path [->, ultra thick] (a) edge (c);
        \path [->, ultra thick] (d) edge (c);
        \path [->, ultra thick] (d) edge (e);
        \path [->, ultra thick] (f) edge (e);
        \path [->, ultra thick] (f) edge (h);
        \path [->, ultra thick] (i) edge (h);
        \path [->, ultra thick] (c) edge (b);
        \path [->, ultra thick] (e) edge (g);
        \path [->] (x1) edge (a);
        \path [->] (a) edge (x2);
        \path [->] (x3) edge (b);
        \path [->] (b) edge (x4);
        \path [->] (b) edge (x5);
        \path [->] (c) edge (x6);
        \path [->] (e) edge (x7);
        \path [->] (g) edge (x8);
        \path [->] (g) edge (x9);
        \path [->] (x10) edge (g);
        \path [->] (h) edge (x11);
        \path [->] (h) edge (x12);
        \path [->] (i) edge (x13);
        \path [->] (x14) edge (i);
        \path [->] (x15) edge (i);
        \path [->] (x16) edge (f);
        \path [->] (x17) edge (f);
        \path [->] (x18) edge (d);
        \path [->] (x19) edge (d);
        \path [->] (x20) edge (a);
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=a--c--b};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=g--e--f};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x1--a--x2};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x3--b--x4};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x5--b--c};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x6--c--d};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=d--e--x7};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=e--g--x8};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x9--g--x10};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=f--h--x11};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x12--h--i};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x13--i--x14};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x15--i--h};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=h--f--x16};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x17--f--e};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=e--d--x18};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x19--d--c};
    	\draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=c--a--x20};
	  \end{tikzpicture}};
\end{tikzpicture}

==> figures/gridQuiver.tex <==
\begin{tikzpicture}[scale=1.4]
    \node[inner sep = 1pt] (a) at (1,3) {$\bullet$};
    \node[inner sep = 1pt] (b) at (2,3) {$\bullet$};
    \node[inner sep = 1pt] (c) at (1,2) {$\bullet$};
    \node[inner sep = 1pt] (d) at (2,2) {$\bullet$};
    \node[inner sep = 1pt] (e) at (3,2) {$\bullet$};
    \node[inner sep = 1pt] (f) at (4,2) {$\bullet$};
    \node[inner sep = 1pt] (g) at (2,1) {$\bullet$};
    \node[inner sep = 1pt] (h) at (3,1) {$\bullet$};
    \node (x1) at (.2,3) {};
    \node (x2) at (.2,2) {};
    \node (x3) at (1,1.2) {};
    \node (x4) at (1.2,1) {};
    \node (x5) at (2,.2) {};
    \node (x6) at (3,.2) {};
    \node (x7) at (3.8,1) {};
    \node (x8) at (4,1.2) {};
    \node (x9) at (4.8,2) {};
    \node (x10) at (4,2.8) {};
    \node (x11) at (3,2.8) {};
    \node (x12) at (2.8,3) {};
    \node (x13) at (2,3.8) {};
    \node (x14) at (1,3.8) {};
    \path [->, ultra thick] (a) edge (b);
    \path [->, ultra thick] (c) edge (a);
    \path [->, ultra thick] (d) edge (b);
    \path [->, ultra thick] (c) edge (d);
    \path [->, ultra thick] (d) edge (e);
    \path [->, ultra thick] (e) edge (f);
    \path [->, ultra thick] (g) edge (d);
    \path [->, ultra thick] (h) edge (e);
    \path [->, ultra thick] (g) edge (h);
    \path [->] (x1) edge (a);
    \path [->] (x2) edge (c);
    \path [->] (x3) edge (c);
    \path [->] (x4) edge (g);
    \path [->] (x5) edge (g);
    \path [->] (x6) edge (h);
    \path [->] (h) edge (x7);
    \path [->] (x8) edge (f);
    \path [->] (f) edge (x9);
    \path [->] (f) edge (x10);
    \path [->] (e) edge (x11);
    \path [->] (b) edge (x12);
    \path [->] (b) edge (x13);
    \path [->] (a) edge (x14);
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=c--a--b};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=b--d--c};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=g--d--e};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=e--h--g};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm, ultra thick]{angle=h--e--f};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x14--a--x1};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=a--c--x2};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x3--c--d};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=d--g--x4};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x5--g--h};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x6--h--x7};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x8--f--x9};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x10--f--e};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x11--e--d};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=d--b--x12};
    \draw pic[draw, angle eccentricity=1.2, angle radius=.4cm]{angle=x13--b--a};
\end{tikzpicture}
